Constellation Shaping under Phase Noise Impairment for Sub-THz Communications

The large untapped spectrum in the sub-THz allows for ultra-high throughput communication to realize many seemingly impossible applications in 6G. One of the challenges in radio communications in sub-THz is the hardware impairments. Specifically, phase noise is one key hardware impairment, which is accentuated as we increase the frequency and bandwidth. Furthermore, the moderate output power of the sub-THz power amplifier demands limits on peak to average power ratio (PAPR) signal design. Single carrier frequency domain equalization (SC-FDE) has been identified as a suitable candidate for sub-THz, although some challenges such as phase noise and PAPR still remain to be tackled. In this work, we design a phase noise robust, modest PAPR SC waveform by geometrically shaping the constellation under practical conditions. We formulate the waveform optimization problem in its augmented Lagrangian form and use a back-propagation-inspired technique to obtain a constellation design that is numerically robust to phase noise, while maintaining a relatively low PAPR compared to the conventional waveforms.

==> 0_notepad.tex <==
1.Sub-THz – an enabling technology for ultra high data rates 

2.Phase noise – one of the key challenges 

3.SC-FDE as the candidate waveform

4.Learning the waveform

5.System Model

6.Problem Formulation

7.Trainable constellation

8.Trainable filter

9.AWGN optimal demapper and Neural Demapper

10.Optimization methodology

11.Evaluation setup

12.Results

13.Discussion, conclusions and outlook

==> 2_RelatedWork.tex <==
\label{2_related_work}

Prior work on waveform selection and adaptation considers a set of candidate waveforms depending on the transmission capability of the devices, desired PAPR (Peak to Average Power Ratio) and ACLR (Adjacent Channel Leakage Ratio) conditions, traffic conditions and other criteria. This proves the fact that depending on the conditions, waveform characteristics adaptation is required. 
In [1], a methods for  add selecting the transmit waveform among a plurality of candidates, OFDMA, SCFDM, CDMA, …, according to the capability of the transmitter and receiver (supported PAPR, ACLR, processing capability, …) and in dependency of other parameters like traffic characteristics (light/heavy, burste/continue, eMBB/URLLC, …) and application types. No adaptation of the waveform parameters is considered.
In [2] signaling techniques for adaptive waveform selection were proposed. A plurality of waveforms according to the capability of the transmit point is indicated via grant request. A selection of one candidate from the plurality according to the traffic characteristics is included in the scheduling procedure.

==> 6_EvaluationSetup.tex <==
\begin{figure*}[]
    \centering
    \includegraphics[width=\textwidth]{Figures/Constellations.eps}
    \caption{Learnt constellations under different PAPR targets}
    \label{fig:constellations}
\end{figure*}
The implementation was done in the widely-used machine learning framework Tensorflow and some components from the open-source library for physical layer research – Sionna \cite{Sionna}. We use the automatic differentiation feature and the optimizers to implement the SGD step. Table \ref{sim_table} summarizes the simulation parameters used for the evaluation. The constellation was initialized with a standard-QAM constellation with Gray-labelling.  We train the end-to-end system on a range of $\frac{E_b}{N_0}$ values with uniform sampling at each iteration such that the learnt waveform is robust in the  applicable SNR range for a chosen modulation order. The AWGN noise variance $\sigma^2$ for a certain $\frac{E_b}{N_0}$ is calculated as,
\begin{equation}
    \sigma^2 = \Big[ \Big(\frac{E_b}{N_0}\Big) r M \Big(\frac{N-QN_P}{N+N_{CP}}\Big)\Big]^{-1}
\end{equation}
where $r$ is the code rate. The end-to-end system is trained as an uncoded ($r=1$) system and for evaluation, an outer channel code with 5G NR LDPC was used for computing the BLER of the system. 

% and effective bandwidth ($BW_{eff}$) where 99\% of the power is contained for the trained system. Then the spectral efficiency ($SE$) is calculated as,

% \begin{equation}
%     SE= \frac{(1-BLER)*R}{BW_{eff}}
% \end{equation}
% and $R$ is the data rate given by,
% \begin{equation}
%     R = r M \Big(\frac{N-QN_P}{N+N_{CP}}\Big)\frac{1}{T_s}
% \end{equation}
% where $T_s$ is the symbol duration.

\begin{table}[ht] \caption{Simulation parameters}\label{sim_table}
\begin{tabular}{|l|l|}
\hline
\textbf{Carrier Frequency}                                                        & 120 GHz                                                                    \\ \hline
\textbf{Bandwidth}                                                                 & 3.93 GHz                                                                   \\ \hline
\textbf{Block size$(N)$}                                                           & 4096                                                                          \\ \hline
\textbf{Modulation order $(K)$}                                                    & 6                                                                                  \\ \hline
\textbf{Oversampling factor  $(M)$}                                                 & 4                                                                                     \\ \hline
\textbf{RRC filter span  $(L)$}                                                     & 32 symbols                                                                            \\ \hline
\textbf{RRC roll-off   $(\beta)$}                                                     & 0.3                                                                           \\ \hline
\textbf{CP Ratio   $(N_{CP}/(N+N_{CP}))$}                                           & 7.03125 \%                                                                \\ \hline
\textbf{Tx Phase Noise Model}                                                       & TI LMX2595 @20GHz (upscaled)                                                          \\ \hline
\textbf{Rx Phase Noise Model}                                                       & \begin{tabular}[c]{@{}l@{}}3GPP TR38.803 v14.2.0 \\ UE model 1 (upscaled)\end{tabular} \\ \hline
\textbf{No of. PTRS blocks  $(Q)$}                                                          & 32                                                                                 \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}PTRS symbols per\\ PTRS block $(N_P)$\end{tabular}}& 4                                                                                     \\ \hline
\textbf{PTRS symbols}                                                               & Zadoff-Chu sequences                                                                  \\ \hline\hline
\textbf{PAPR Targets $(\epsilon_p)$}                                                & 6.5dB, 7.0 dB, 7.5 dB, 8.0 dB                                         \\   \hline
%\textbf{ACLR Target}                                                                & -20 dB, -25dB, -35dB for $1+ \beta$                            \\ \hline
%\textbf{Excess bandwidth targets ($\beta$ )}                                               & 0.1, 0.12, 0.15, 0.2, 0.3                                                       \\ \hline
\textbf{Batch size}                                                                 & 10                                                                                    \\ \hline
\textbf{Optimizer}                                                                  & Adam                                                                                  \\ \hline
\textbf{Learning rate}                                                              & 1e-3                                                                                  \\ \hline
\textbf{Training EbN0 range}                                                        & {[}6-18{]} dB                                         \\ \hline
\textbf{EbN0 sampling}                                                              & Uniform                                                                               \\ \hline \hline
\textbf{Evaluation – Channel Code}                                                  & 5G NR LDPC                                                                               \\ \hline
\textbf{Code rate}                                                                  & 3/4                                                                                   \\ \hline
\textbf{BP iterations}                                                              & 50                                                                                    \\ \hline
\end{tabular}
\end{table}
